Semantic Relations and Deep Learning

The second edition of "Semantic Relations Between Nominals" by Vivi Nastase, Stan Szpakowicz, Preslav Nakov and Diarmuid \'O S\'eaghdha has been published in April 2021 by Morgan & Claypool (www.morganclaypoolpublishers.com/catalog_Orig/product_info.php?products_id=1627). A new Chapter 5 of the book, by Vivi Nastase and Stan Szpakowicz, discusses relation classification/extraction in the deep-learning paradigm which arose after the first edition appeared. This is Chapter 5, made public by the kind permission of Morgan & Claypool.

==> morgxml.tex <==
%
\ifx\xmlfile\@undefined%
\else%
  \input isotech.tex
\fi%
%
\def\storetitle#1{}
\def\getlabel#1{\gdef\@getlabel{#1}}
%
\def\getjournalid#1{}
\def\getissn#1{}
\def\getpublisher#1{}
\def\getarticleid#1{}
\def\getalttitle#1{\gdef\@getalttitle{#1}}\getalttitle{}
\def\getarticletitle#1{\gdef\@getarticletitle{#1}}
\def\getcontrib#1{\author{#1}}
\def\getaff#1{\affiliation{#1}}
\def\getpubdate#1{}
\def\getvolume#1{}
\def\getfpage#1{}
\def\getlpage#1{}
\def\getcopyrightstatement#1{}
\def\getcopyrightyear#1{}
%
\def\getcaption#1{\protected@xdef\@CAPTION{#1}}

%
%%%%%%%% BIBLIOGRAPHY
%
\def\activatereftags{%
   \let\getaccessdate\getbib@accessdate%
   \let\getannotation\getbib@annotation%
   \let\getarticletitle\getbib@articletitle%
   \let\getcollab\getbib@collab%
   \let\getcomment\getbib@comment%
   \let\getconfdate\getbib@confdate%
   \let\getconfloc\getbib@confloc%
   \let\getconfname\getbib@confname%
   \let\getday\getbib@day%
   \let\getedition\getbib@edition%
   \let\getemail\getbib@email%
   \let\getelocationid\getbib@elocationid%
   \let\getetal\getbib@etal%
   \let\getfpage\getbib@fpage%
   \let\getgov\getbib@gov%
   \let\getissn\getbib@issn%
   \let\getisbn\getbib@isbn%
   \let\getissue\getbib@issue%
   \let\getlpage\getbib@lpage%
   \let\getmonth\getbib@month%
   \let\getname\getbib@name%
   \let\getpatent\getbib@patent%
   \let\getpersongroup\getbib@persongroup%
   \let\getpubid\getbib@pubid%
   \let\getpublisherloc\getbib@publisherloc%
   \let\getpublishername\getbib@publishername%
   \let\getseason\getbib@season%
   \let\getseries\getbib@series%
   \let\getsource\getbib@source%
   \let\getstd\getbib@std%
   \let\getsupplement\getbib@supplement%
   \let\gettimestamp\getbib@timestamp%
   \let\gettranssource\getbib@transsource%
   \let\gettranstitle\getbib@transtitle%
   \let\getvolume\getbib@volume%
   \let\getyear\getbib@year%
}
%
\def\getbib@accessdate#1{#1}
\def\getbib@annotation#1{#1}
\def\getbib@articletitle#1{#1}
\def\getbib@collab#1{#1}
\def\getbib@comment#1{#1}
\def\getbib@confdate#1{#1}
\def\getbib@confloc#1{#1}
\def\getbib@confname#1{#1}
\def\getbib@day#1{#1}
\def\getbib@edition#1{#1}
\def\getbib@email#1{#1}
\def\getbib@elocationid#1{#1}
\def\getbib@etal#1{#1}
\def\getbib@fpage#1{#1}
\def\getbib@gov#1{#1}
\def\getbib@issn#1{#1}
\def\getbib@isbn#1{#1}
\def\getbib@issue#1{#1}
\def\getbib@lpage#1{#1}
\def\getbib@month#1{#1}
\def\getbib@name#1{#1}
\def\getbib@patent#1{#1}
\def\getbib@persongroup#1{#1}
\def\getbib@pubid#1{#1}
\def\getbib@publisherloc#1{#1}
\def\getbib@publishername#1{#1}
\def\getbib@season#1{#1}
\def\getbib@series#1{#1}
\def\getbib@source#1{#1}
\def\getbib@std#1{#1}
\def\getbib@supplement#1{#1}
\def\getbib@timestamp#1{#1}
\def\getbib@transsource#1{#1}
\def\getbib@transtitle#1{#1}
\def\getbib@volume#1{#1}
\def\getbib@year#1{#1}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Tables %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcount\colcount%
\def\getCOLNUM#1#2{%
\global\colcount\expandafter\getnumber#2%
\global\advance\colcount-\expandafter\getnumber#1%
\global\advance\colcount1%
}%
%
\def\getnumber col#1{#1}%
%
\gdef\base{10pt}%%for table body leading
\gdef\colbase{10pt}%%for table column head leading
\newif\ifhangtab\global\hangtabfalse
%
\newcount\tfootcount
\global\tfootcount0
%
\def\tablefootnote#1#2{%\expandafter\gdef\csname affiliation\the\affiliationcount\endcsname{#1}%
        \global\advance\tfootcount1\expandafter\gdef\csname tablefootnote\the\tfootcount\endcsname{#2}}
%
\def\showtfoot{\let\getlabel\gettfootlabel\global\tempcount0
%               \vskip-2.5pt%
%               \ifdim\tablewidth>\textheight%
%                 \vskip-7.5pt\centerline{\hskip11pt\vrule width\tablewidth height.5pt\hskip-11pt}\vskip-4pt
%               \else%
%                 \vskip-7.5pt\centerline{\vrule width\tablewidth height.5pt}\vskip-4pt
%               \fi%
                 \@whilenum\tempcount<\tfootcount
   						        \do{%
%                 				\color{\Bcolorthree\hskip0pt\csname tablefootnote\the\tempcount\endcsname\endgraf}
                 				\hskip0pt\csname tablefootnote\the\tempcount\endcsname\endgraf%
                     \global\advance\tempcount1}%
%               and\ \csname author\the\tempcount\endcsname%
            %
  }
%
\newif\ifframed\framedfalse
\newif\ifnotablenum
%
\def\tablebodystartleftskip#1{\gdef\@tablebodystartleftskip{#1}}\tablebodystartleftskip{9pt}
\def\tablebodystartrightskip#1{\gdef\@tablebodystartrightskip{#1}}\tablebodystartrightskip{9pt}
%
%
%\def\interfootnote{\vphantom{PQpqfg}\\[-\baselineskip]}
%
\def\gettfootlabel#1{#1}
%
%\def\morgan@footnote#1#2{\protected@write\@mainfnnote{}%
%{<fn-link id="#1">#2<?TeX \vspace*{-\baselineskip}?></fn-link>}%
%}
%
\def\XREF#1{#1}
%
\def\DispQuotetitle#1{#1}
%
\newenvironment{DispQuote}{\par\let\storetitle\DispQuotetitle}{\par}
%

